PRISM: : Planning and Reasoning with Intent in Simulated Embodied Environments

When an LLM-based embodied agent fails at a household task, the culprit could be misidentified objects, forgotten sub-goals, or poor action sequencing -- yet existing benchmarks report only a single success rate, making it impossible to tell which cognitive module is responsible. We present PRISM, a diagnostic benchmark that reframes this problem: rather than asking only \textit{did the agent succeed?}, PRISM asks \textit{which capability is most likely responsible for failure?} Built on five photorealistic multi-room apartments (4--8 rooms each), PRISM structures 300 human-verified tasks into three capability tiers -- \textit{Basic Ability}, \textit{Reasoning Ability}, and \textit{Long-horizon Ability} -- that isolate perception-to-action grounding, implicit intent resolution, and sustained multi-step coordination respectively. PRISM exposes an agent-agnostic executable action API that allows arbitrary agents: LLM agents, VLM agents, symbolic planners, RL policies, and hybrid systems, to be evaluated end-to-end under the same benchmark protocol. To support deeper diagnosis, optional probes for perception, memory, and planning can be adopted, replaced, or bypassed entirely, enabling controlled component-level analysis when desired. Experiments on seven contemporary LLMs establish a clear hierarchy: explicit spatial grounding is not the dominant failure source under oracle perception, implicit intent resolution is a significant bottleneck for all model families, and long-horizon coordination exposes a stark capability cliff -- lightweight models collapse to as low as 20.0\% success while simultaneously consuming more tokens than their frontier counterparts, a signature of compensatory over-reasoning rather than genuine planning capability. Project page: \href{https://sj-li.com/PROJ/PRISM}{link}.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction explicitly state three contributions (diagnostic benchmark, modular pipeline, scene-graph task generation) and scope them to household embodied planning under oracle perception. Experimental results in Section~5 directly support all three claims, and the Limitations paragraph in Section~6 clarifies scope boundaries.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: A dedicated Limitations paragraph in Section~6 (Conclusion) discusses oracle-only perception, five-scene scope, LLM task generation bias, simulator asset bias, and household-only coverage. Extended discussion appears in Appendix~\ref{sec:supp_limitations}.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper contains no theoretical results or proofs. The formalization in Section~3.1 (Eq.~1) is a standard MDP-style notation used to define the evaluation setting, not a theorem.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~5 specifies all evaluated models (with citations), the oracle perception setting, and identical prompt usage. Appendix~\ref{sec:supp_impl} provides all hyperparameters (temperature=0.0, step budget=60, memory window=10). The simulator uses deterministic physics, so identical action sequences reproduce identical outcomes. Prompt templates are in Appendix~\ref{sec:supp_prompt}.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: An anonymized GitHub repository is provided with the submission containing the simulator binary, 300-task JSON dataset, evaluation scripts, scene configurations, and prompt templates. See Appendix~\ref{sec:supp_artifact} for full release documentation.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: No training is performed; \prism is a pure evaluation benchmark. All evaluation hyperparameters (temperature, step budget, memory window size, interaction range, parallel instances, API endpoint) are reported in Appendix~\ref{sec:supp_impl}. The 300-task evaluation set is fixed and fully released.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Error bars are not reported for the main results, as each model is evaluated on the full fixed 300-task set under deterministic decoding (temperature=0.0), eliminating run-to-run variance. Per-apartment SR breakdown (Table~4) provides a measure of result consistency across scene layouts (std=2.5\%).

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All experiments use LLM APIs via OpenRouter (no local GPU required). The simulator runs on CPU with 8 parallel instances (Appendix~\ref{sec:supp_impl}). Compute cost is dominated by API token consumption, which is reported as Token Count (TC) in Table~\ref{tab:main_results}; for example, GPT-5.2 consumes 58.4K, 100.6K, and 126.8K tokens on average per task on Basic, Reasoning, and Long-horizon tasks, respectively.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification: This work introduces an evaluation benchmark for embodied AI agents in simulated household environments. It involves no human subjects research, no sensitive data collection, no deployment of systems with societal risk, and no dual-use concerns. The benchmark assets are licensed for academic research use.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Positive impact: enabling more targeted improvement of embodied AI systems by attributing failures to specific cognitive modules, accelerating progress toward assistive household robots. Negative impact: benchmark-driven optimization could produce agents that perform well on \prism's household scenarios without generalizing to real-world diversity (Goodhart's Law); this is discussed in the Limitations paragraph of Section~6.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: \prism releases a simulation environment and task dataset, not a pre-trained model or scraped dataset. The benchmark poses no meaningful misuse risk beyond general embodied AI research; no special safeguards are required. See Appendix~\ref{sec:supp_limitations} for responsible use discussion.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: Unity 6 (Unity Technologies, standard EULA), Unity ML-Agents (Apache 2.0), and all LLM APIs (accessed under commercial terms of service) are cited. Third-party 3D assets are licensed for academic research use; license documentation is included in the released repository (Appendix~\ref{sec:supp_artifact}).

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: \prism introduces a new benchmark comprising a simulator binary, 300-task JSON dataset, scene configurations, and evaluation scripts. Full documentation is in Appendix~\ref{sec:supp_artifact}, covering release contents, reproducibility guarantees, license terms, and the rationale for using an executable environment format rather than a static dataset format.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Human feasibility verification is described in Section~3.3 and Appendix~\ref{sec:supp_taskgen}. Annotators executed each task in the simulator using a keyboard interface and assessed three criteria (executability, instruction clarity, object reachability). The human evaluation study (Appendix~\ref{sec:supp_ablation}) used the same interface. Participants were internal lab members. No external crowdsourcing platform was used. Participation involved only interacting with a simulator interface; no sensitive personal data were collected. No separate compensation beyond normal institutional arrangements was provided.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The human evaluation involved lab members interacting with a video game-like simulator interface. No physical risk, sensitive data collection, or deception was involved. IRB review was not required under our institution's guidelines for this type of low-risk internal evaluation.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerYes{}
    \item[] Justification: LLMs are the primary evaluated agents in this benchmark paper, and their usage is described throughout. Specifically: (1) LLMs are used as the Memory and Planning modules during evaluation (Section~4); (2) an LLM is used during task generation (Section~3.3, Appendix~\ref{sec:supp_taskgen}); (3) all evaluated models (GPT-5.2, Claude Sonnet~4.6, Gemini~3~Flash, GLM-4.6V, and lightweight variants) are cited with their respective technical reports.

\end{enumerate}

